Memory-Efficient Federated Fine-Tuning of Large Language Models via Layer Pruning

Federated fine-tuning enables privacy-preserving Large Language Model (LLM) adaptation, but its high memory cost limits participation from resource-constrained devices. We propose FedPruner, an innovative federated fine-tuning paradigm that tackles this via intelligent layer pruning. FedPruner flexibly prunes the global model, creating personalized submodels based on device memory constraints. It employs a macro-micro synergistic pruning framework: a macro-level functionality-driven layer orchestration mechanism groups layers, while a micro-level importance-aware layer selection strategy prunes within groups to build device-specific submodels. We further introduce a fine-grained variant that independently prunes Multi-Head Attention and Feed-Forward Network components to precisely preserve critical architectural elements. Extensive experimental results demonstrate that FedPruner significantly outperforms state-of-the-art approaches, achieving up to a 1.98\% improvement in average model accuracy while reducing peak memory usage by 75\%.

==> Section/Preliminary.tex <==
\section{Preliminary}



In this section, we introduce how to effectively fine-tune LLMs using LoRA~\cite{hu2021lora}.
The core concept of LoRA involves updating model parameters through low-rank matrix decomposition while maintaining the original model weights frozen.
Figure~\ref{lora_module} illustrates the working principle of LoRA, wherein the pre-trained weight matrix $\mathbf{W}_{0} \in \mathbb{R}^{U_{1}\times U_{2}}$ remains frozen while its update $\mathbf{\Delta W}$ is parameterized through a low-rank factorization. Specifically, $\mathbf{\Delta W}$ is factorized into the product of two trainable matrices $\mathbf{B} \in \mathbb{R}^{U_{1}\times r}$ and $\mathbf{A} \in \mathbb{R}^{r\times U_{2}}$, with rank $r$ significantly smaller than $\min(U_{1},U_{2})$.
The input is processed in parallel by both $\mathbf{W}_{0}$ and $\mathbf{\Delta W}$, with their outputs merged via element-wise addition. For a linear layer $h = \mathbf{W}_{0}x$, the modified forward propagation is formulated as: $h = \mathbf{W}_{0}x + \mathbf{B}\mathbf{A}x$.

\begin{wrapfigure}{r}{0.27\textwidth}
\vspace{-15pt}
\centering
\adjustbox{max width=0.27\textwidth}{\includegraphics{Graph/LoRA_pre.pdf}}
\vspace{-7pt}
\caption{The working principle of LoRA.}
\label{lora_module}
\vspace{-10pt}
\end{wrapfigure}
Compared to full-parameter fine-tuning, LoRA significantly reduces the number of trainable parameters by only updating the low-rank matrices. After completing local fine-tuning, devices only need to upload the LoRA parameters to the server, substantially reducing the communication overhead. 
The central server then aggregates these updates from the participating device set $S$ using the stacking-based aggregation strategy~\cite{wang2024flora}, as formulated in Equation~\eqref{eq_flora}.
Here, $\lambda_{s}$ denotes the scaling factor, calculated as $\lambda_{s} = \frac{|D_{s}|}{\sum_{s=1}^{|S|}|D_{s}|}$, where $|D_{s}|$ represents the local dataset size of device $s$, and “$\oplus$” represents the stacking operation: vertical stacking for matrix $\mathbf{A}$ and horizontal stacking for matrix $\mathbf{B}$.
\begin{equation}
\small
\begin{split}
    \mathbf{A} &= \lambda_{1}\mathbf{A}_{1} \oplus \lambda_{2}\mathbf{A}_{2}\oplus \cdots \oplus \lambda_{|S|}\mathbf{A}_{|S|}, \\
    \mathbf{B} &= \mathbf{B}_{1} \oplus \mathbf{B}_{2}\oplus \cdots \oplus \mathbf{B}_{|S|}.
\end{split}
\label{eq_flora}
\end{equation}


==> Table/Table_Overhead.tex <==
\definecolor{steelblue}{HTML}{82B0D2}
\definecolor{my_c1}{HTML}{aacfd0}

\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule[1pt]
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Resource Consumption ($\downarrow$)}}\\  

\cmidrule{2-3}

& \textbf{Time (h)} & \textbf{Communication (GB)} \\ 
\midrule[1pt]
FedIT & 3.22 & 6.05 \\
DoFIT & 4.48 & 7.62\\
FedSA-LoRA & 2.93 & 5.46\\
FLoRA & 3.61 & 7.46\\
FwdLLM & 2.98 & 5.58\\
FedRA & 2.10 & 3.65 \\
Full LoRA$^\dagger$ & 2.56 & 5.03\\
\midrule[0.5pt]
\rowcolor{my_c1!50}
FedPruner & \textbf{1.92} & \textbf{3.47} \\
\bottomrule[1pt]
\end{tabular}
}

==> Table/table2_ablation.tex <==
\definecolor{steelblue}{HTML}{82B0D2}
% \definecolor{my_c1}{HTML}{a4e5d9}
\definecolor{my_c1}{HTML}{aacfd0}
% \begin{table}[!t]
% \caption{\textbf{Ablation study of \texttt{\textbf{FedPruner}}.} }
% \vspace{2pt}
% \small
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule[1pt]
\multirow{2}{*}{\textbf{Method}}  & \multicolumn{4}{c}{\textbf{Close-Ended Benchmark}} &\multirow{2}{*}{\textbf{Average}} \\  

\cmidrule{2-5}

& \textbf{TruthfulQA} & \textbf{MMLU} & \textbf{IFEval} & \textbf{BBH}   \\ 
\midrule[1pt]
&\multicolumn{4}{c}{\textbf{LLaMA2-7B (INT4)}} &\\ 
\midrule[1pt]
\rowcolor{my_c1!70}
FedPruner & \textbf{49.95} & \textbf{43.64} & \textbf{33.72} & \textbf{40.65} & \textbf{41.99} \\
w/o FDLO                    & 48.14 & 42.93 & 32.44 & 39.58 & 40.77 \\ 
w/o IALS                    & 49.38 & 43.02 & 32.87 & 40.42 & 41.42 \\
w/o FDLO \& IALS & 47.66 & 42.41 & 31.67 & 39.36 & 40.28\\

\midrule[1pt]
&\multicolumn{4}{c}{\textbf{LLaMA2-13B (INT4)}} &\\ 
\midrule[1pt]
\rowcolor{my_c1!70}
FedPruner & \textbf{56.13} & \textbf{58.09} & \textbf{45.62} & \textbf{48.46} & \textbf{52.08} \\
w/o FDLO                    & 53.24 & 55.76 & 41.47 & 46.45 & 49.23  \\ 
w/o IALS                    & 54.82 & 56.94 & 43.64 & 47.74 & 50.79  \\
w/o FDLO \& IALS & 51.69 & 54.93 & 39.11 & 45.39 & 47.78 \\
\bottomrule[1pt]
\end{tabular}
}
% \label{ablation_study}
% \vspace{-6mm}
% \end{table}

==> Table/table_sensitivity.tex <==
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule[1pt]
\multirow{2}{*}{\textbf{Interval}}  & \multicolumn{2}{c}{\textbf{Global Model}} \\  

\cmidrule{2-3}

&LLaMA2-7B & LLaMA2-13B \\ 
\midrule[1pt]
$T=1$& \textbf{43.64} & \textbf{58.09}\\ 
$T=10$& 43.41 & 57.73 \\ 
$T=20$& 43.06 & 57.38\\ 
$T=50$& 42.68 & 56.62 \\ 
\bottomrule[1pt]
\end{tabular}
}

